Beyond Convolutions: A Novel Deep Learning Approach for Raw Seismic Data Ingestion

Traditional seismic processing workflows (SPW) are expensive, requiring over a year of human and computational effort. Deep learning (DL) based data-driven seismic workflows (DSPW) hold the potential to reduce these timelines to a few minutes. Raw seismic data (terabytes) and required subsurface prediction (gigabytes) are enormous. This large-scale, spatially irregular time-series data poses seismic data ingestion (SDI) as an unconventional yet fundamental problem in DSPW. Current DL research is limited to small-scale simplified synthetic datasets as they treat seismic data like images and process them with convolution networks. Real seismic data, however, is at least 5D. Applying 5D convolutions to this scale is computationally prohibitive. Moreover, raw seismic data is highly unstructured and hence inherently non-image like. We propose a fundamental shift to move away from convolutions and introduce SESDI: Set Embedding based SDI approach. SESDI first breaks down the mammoth task of large-scale prediction into an efficient compact auxiliary task. SESDI gracefully incorporates irregularities in data with its novel model architecture. We believe SESDI is the first successful demonstration of end-to-end learning on real seismic data. SESDI achieves SSIM of over 0.8 on velocity inversion task on real proprietary data from the Gulf of Mexico and outperforms the state-of-the-art U-Net model on synthetic datasets.

==> application.tex <==



% \begin{figure*}
% \begin{subfigure}{.35\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/overfitting/ssim.png}
%   \caption{Test SSIM}
%   \label{fig:overfit1}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/overfitting/psnr.png}
%   \caption{Test PSNR}
%   \label{fig:overfit2}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/overfitting/l1.png}
%   \caption{Test L1 loss}
%   \label{fig:overfit3}
% \end{subfigure}
% \caption{The figure evolution of metrics SSIM, L1 loss and PSNR on test SEGSalt dataset as the training progresses to 1200 epochs. As can be seen SSIM always improves and L1 loss , PSNR achieve stable values. For elaboration on metrics see Experiments section.}
% \label{fig:overfit}

% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/fractionalsample/f_ssim.png}
%   \caption{Test SSIM}
%   \label{fig:frac1}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/fractionalsample/f_psnr.png}
%   \caption{Test PSNR}
%   \label{fig:frac2}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figures/fractionalsample/f_l1.png}
%   \caption{Test L1 loss}
%   \label{fig:frac3}
% \end{subfigure}
% \caption{Model is trained with 0.8 fraction of traces. Comparison on test performance when different fractions of traces is used for inference}
% \label{fig:frac}

% \end{figure*}
\vspace{-0.2cm}
\section{Application and Empirical Results}
\vspace{-0.2cm}


\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Method          & subsample & $l_1$ loss      & PSNR           & SSIM          \\ \hline
U-Net           & -         & 196.82          & 14.64          & 0.45          \\ \hline
Set Transformer & -         & 232.78          & 14.21          & 0.40          \\ \hline
Set Transformer & 50\%      & 294.76          & 14.90          & 0.34          \\ \hline
SESDI           & -         & 163.77          & 16.65          & \textbf{0.47} \\ \hline
SESDI           & 50\%      & \textbf{162.79} & \textbf{16.86} & 0.41          \\ \hline
\end{tabular}
}
\caption{Evaluation Metrics on SEGSalt Data for different SDI approaches on Velocity Inversion problem.}
\label{tab:eval-sim}
\vspace{-0.6cm}
\end{table}
\begin{figure}
    \centering
    \includegraphics[scale=0.55]{figures/syntheticacquision.png}
    \caption{Regular AG used in synthetic datasets is to have sources and receivers uniformly distributed on surface and have every receiver listen to every source. Realistic AG for 2D is designed to mimic Real acquisition. Here, randomly sampled contiguous segments of receivers are made to listen to each source. }
    \label{fig:syntheticAQ}
\end{figure}

\input{img_fract_overfit}

We apply SESDI model on the velocity inversion problem to showcase its utility. The experiments are divided into two major subcategories. 
\textbf{1.Baselines:} A) comparison with state-of-the art U-net model and another set based model, set transformer \cite{lee2019set} on synthetic 2D VMB problem using regular acquistion data.   
B) We modify the acquisition geometry of synthetic datasets to resemble real acquisition. We show the robustness of SESDI w.r.t irregular and inconsistent acquisition geometry as claimed above and compare against \cite{lee2019set}.

\textbf{2. Experiments on Real data:} We provide the first ever results on real data from Gulf of Mexico at its original scale for problem of Velocity Inversion. 

\textbf{Metrics:} To evaluate the trained models, we use three major metrics for evaluation: $\ell_1$ Loss (lower is better) , PSNR~\cite{huynh2008scope}(higher is better) and SSIM~\cite{wang2004image}(higher is better, which are widely utilized by recent  literature~\cite{Yang2019Deeplearning,inversionnet,rojas2020physics,araya2018deep}.

%We present a set of scenarios for our SESDI model. For simulation setting, we compare the SESDI model with state-of-the-art U-Net model on 2D VMB. Moreover, we evaluate SESDI model's scalability and sustainability in 3D VMB with raw seismic data as input, where CNN based deep learning methods are prohibited due to oversimplified acquisition geometry assumptions. 
\vspace{-0.2cm}
\subsection{2D Velocity Inversion on Synthetic Data}
%\vspace{-0.2cm}
%\subsubsection{Settings}
%\vspace{-0.1cm}
{\bf Benchmark Dataset} We use SEGSalt dataset~\footnote{https://wiki.seg.org/wiki/SEG} provided by \cite{Yang2019Deeplearning}. SEGSalt is one of the largest publicly available for velocity inversion dataset. Authors of \cite{Yang2019Deeplearning} generate the synthetic traces in SEGSalt by first obtain a 2D velocity slices and then performing acoustic wave equation based forward modelling to generate seismic gathers using tools such as devito \cite{devito-api, devito-compiler}. The details of setup is provided in appendix \ref{apx:sim}. \\
{\bf Baseline:} The network architecture and training strategy for SESDI, U-net and set transformer is provided in appendix \ref{apx:net} and \ref{apx:train}. 

%We use two types of velocity models dataset for 2D VMB: 2D simulated models and 2D SEGSalt models extracted from a 3D salt model~\footnote{https://wiki.seg.org/wiki/SEG}. To the best of our knowledge, these two datasets are considered as the largest datasets publicly available for VMB. Given both synthetic and real velocity model, we perform the acoustic wave equation to generate traces follow the same parameters as~\cite{Yang2019Deeplearning} , details of simulation are shown in Appendix ~\ref{apx:sim}. Then the synthetic traces and their corresponding 2D velocity matrices form data-label pairs. The network architecture as well as the training strategy of SESDI and U-Net is presented in Appendix~\ref{apx:net} and~\ref{apx:train}. 

\vspace{-0.2cm}
\subsubsection{Results}
\vspace{-0.2cm}

\input{img_vissegsalt}


In this section, we present the performance of SESDI, UNet and SetTransformer on SEGSalt dataset From Table~\ref{eval:sim}, we observe that SESDI outperforms state-of-the art U-Net and other set-based model baseline in all three evaluation metrics. The comparison of SESDI, U-Net prediction and ground-truth velocity matrices are shown in Figure~\ref{fig:salt_demo}. Visualization of entire test set are presented in Appendix~\ref{apx:sim_vis}, Figure~\ref{fig:salt}. As shown in figures, we observe that U-Net which aims to learn the shape of the salt body, suffers from two major drawbacks: (1) the prediction of background velocities is less focused, (2) the mis-modeling on the salt body leads to significant performance drop as salt body has the highest velocity. On the contrary, SESDI outperforms U-Net by its clearer characterization on the background and less mis-modeling on salt bodies. We also verify, the intuition that our model does not over fit on scarce data. SEGSalt training dataset has 130 samples. While training, we run each epoch by subsampling 0.8 fraction of traces. Hence, essentially, we are able to train with much larger number of samples. Then, we evaluate on test traces with same subsample rate. As can be seen from Figure\ref{fig:frac_overfit}, that SESDI based model does not overfit even after training for 1200 epochs.

% \begin{figure*}[]
% \centering % <-- added
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_0.png}
%   \caption{gisette}
%   \label{fig:1}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_1.png}
%   \caption{epsilon}
%   \label{fig:2}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_2.png}
%   \caption{cifar10}
%   \label{fig:3}
% \end{subfigure}

% %\medskip
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_3.png}
%   \caption{sector}
%   \label{fig:4}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_4.png}
%   \caption{rcv1}
%   \label{fig:5}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.6\textwidth}
%   \includegraphics[width=\linewidth]{figures/SEGSalt/Vis_5.png}
%   \caption{}
%   \label{fig:6}
% \end{subfigure}
% \caption{}
% \vspace{-0.5cm}
% \label{fig:f1max}
% \end{figure*}


%\begin{table*}[h]
%\begin{center}
%\setlength{\abovecaptionskip}{3pt}
%\setlength{\belowcaptionskip}{2pt}
% \caption{Evaluation Metrics on Sythetic Data}
% \begin{tabular}{ p{2cm}|p{2.5cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm} }
% \hline
% Dataset &   Method & Subsample& $\ell_1$ Loss& PSNR & SSIM   \\
% \hline\hline
%SEGSalt & U-Net & None &196.8229 & 14.6458 & 0.4543   \\
%SEGSalt & Set Transformer& None & 232.7822 & 14.2083 & 0.3968   \\
%SEGSalt & Set Transformer& 50$\%$ & 294.7577 & 14.9020 & 0.3400   \\
%SEGSalt & SESDI &None& 163.7738 & 16.6513 & \textbf{0.4676}   \\
%SEGSalt & SESDI &50$\%$& \textbf{162.7882} & \textbf{16.8633} & 0.4110   \\
% Nakika50 & SESDI  &None& 135.2780 & 32.3479 & 0.8182   \\
% Nakika100 & SESDI &None& 164.9949 & 26.9546 & 0.7462   \\

%Simulation & U-Net & 112.3068 & 24.0570 & 0.4655   \\
%Simulation & SESDI & 164.0342 & 16.6349 & 0.4696   \\
% \hline
 
%\end{tabular}\label{eval:sim}
%\end{center}
%\end{table*}

\vspace{-0.2cm}
\subsection{Realistic Acquisition on Synthetic 2D Data} % @zhaozhuo ablation study means you measure impact of each component in the system by removing it . This is not applicable here
\vspace{-0.2cm}

In order to show the robustness of SESDI over irregular and inconsistent acquisition geometry, we sub-sample the traces from synthetic data in a manner to resemble realistic acquisition. This is shown in figure \ref{fig:syntheticAQ}.  The Figure \ref{fig:frac_overfit} shows the stability of SESDI when fed with varying amounts of irregularly acquired traces on SEGSalt data. As stated earlier, U-net models cannot be applied to such a data. In Table~\ref{tab:eval-sim}, it is shown that SESDI with irregular 50$\%$ of sub-sampling outperforms U-Net with regular observation. 
 %\begin{figure*}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/fractionalsample/f_ssim.png}
%  \caption{Test SSIM}
%  \label{fig:frac1}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/fractionalsample/f_psnr.png}
%  \caption{Test PSNR}
%  \label{fig:frac2}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/fractionalsample/f_l1.png}
%  \caption{Test L1 loss}
%  \label{fig:frac3}
%\end{subfigure}
%\caption{Model is trained with 0.8 fraction of traces. Comparison on test %performance when different fractions of traces is used for inference}
%\label{fig:frac}
%\end{figure*}


% \begin{figure*}[htb]
% \begin{center}
%  \mbox{\hspace{-0.2in}
%  \includegraphics[width=1in]{figures/nakika100/label4.jpg}
% \includegraphics[width=1in]{figures/nakika100/label28.jpg}
% \includegraphics[width=1in]{figures/nakika100/label44.jpg}
% \includegraphics[width=1in]{figures/nakika100/label71.jpg}
% \includegraphics[width=1in]{figures/nakika100/label84.jpg}
%     }
% \mbox{\hspace{-0.2in}
%  \includegraphics[width=1in]{figures/nakika100/output4.jpg}
% \includegraphics[width=1in]{figures/nakika100/output28.jpg}
% \includegraphics[width=1in]{figures/nakika100/output44.jpg}
% \includegraphics[width=1in]{figures/nakika100/output71.jpg}
% \includegraphics[width=1in]{figures/nakika100/output84.jpg}
%     }
% \mbox{\hspace{-0.2in}
% \includegraphics[width=4in]{figures/nakika50/bar.pdf}
% }

% \end{center}

% \vspace{-0.15in}
% \caption{Visualization of Prediction on Nakika100 Dataset. Top: ground-truth velocity cube, Bottom: predicted velocities }\label{fig:nakika100_demo}
% \end{figure*}







\vspace{-0.2cm}
\subsection{3D Velocity Inversion on Real Raw Seismic Data}
\vspace{-0.2cm}

In this section, we show an experiment on large scale 3D VMB performed with one of the major energy and petrochemical company using real raw gather data from Gulf of Mexico (\cite{crout2008oil}). We use proprietary velocity model obtained from traditional approaches to train and test SESDI model.
To the best of our knowledge, this experiment is the first veocity inversion on real seismic data. In this scenario, data is high dimensional (5D) and the acquisition geometry is not regular and consistent like Synthetic data. Therefore, the CNN methods such as U-Net cannot be applied.
\vspace{-0.2cm}
\subsubsection{Training Data Generation}
\vspace{-0.2cm}

In accordance with the methodology specified in section \ref{sec:approach}, we generate data samples $(\mathcal{C}(q, w), \mathcal{P}(q, w_p, d))$ with $w_p=1km$ and $w=5km$  We choose two values for d to generate two different datasets. One predicts velocity block with depth 10\% (Nakika50) and other 20\% (Nakika100) of total depth of real velocity model . The discretized velocity block for Nakika50 is of dimension $17 \times 20 \times 50$ and that for Nakika100 is $17 \times 20 \times 100$. Details about this dataset are presented in Appendix~\ref{apx:nakika}. Nakika50 and Nakika100 datasets have size over 107G and 115G respectively. For each velocity cubes in both dataset, the number of corresponding traces in context varies from $2$ to $8779$.

% \begin{figure}[htb]
% \begin{center}
%  \mbox{\hspace{-0.2in}

% \includegraphics[width=2.5in]{figures/large/large.pdf}}
% \mbox{\hspace{-0.2in}
% \includegraphics[width=2.2in]{figures/nakika50/bar.pdf}
% }

% \end{center}

% \vspace{-0.15in}
% \caption{Combined Visualization  }\label{fig:large_area}
% \end{figure}

%We provide experiment on two dataset: Nakika50 and Nakika100, from the field survey of one major energy and petrochemical company by Nakika platform~\cite{crout2008oil}. The major difference of these two datasets is that Nakika50's velocity matrices are in shape  $17\times20\times50$ while Nakika100 has matrices with shape $17\times20\times100$. To the best of our knowledge, this experiment is the first VMB modeling on real seismic datasets. Details about this dataset are presented in Appendix~\ref{apx:nakika}. Nakika50 and Nakika100 datasets have size over 107G and 115G. For each velocity cubes in both dataset, the number of corresponding traces varies from $2$ to $8779$. Therefore, the Nakika datasets are in a set format that prohibited convolution models.  We use the same three metrics as synthetic dataset.


\begin{table}[]
\begin{center}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{2pt}
 \caption{SESDI on Nakika Data}
 \begin{tabular}{ p{1.8cm}|p{1.2cm}|p{1cm}|p{1cm} }
 \hline
 Dataset &  $\ell_1$ Loss& PSNR & SSIM   \\
 \hline\hline
Nakika50 &    135.2780 & 32.3479 & 0.8182   \\
Nakika100 &  164.9949 & 26.9546 & 0.7462   \\

%Simulation & U-Net & 112.3068 & 24.0570 & 0.4655   \\
%Simulation & SESDI & 164.0342 & 16.6349 & 0.4696   \\
 \hline
 
\end{tabular}\label{eval:sim}
\end{center}
\vspace{-0.2cm}
\end{table}

\vspace{-0.2cm}
\subsubsection{Results}
\vspace{-0.2cm}

 From Table~\ref{eval:sim}, we observe that SESDI achieves promising performance on three evaluation metrics. The comparison of SESDI with ground-truth velocity matrices for Nakika100 is shown in  Figure~\ref{fig:nakika100_demo}. We defer the Nakika50 results to  Appendix (~\ref{apx:sim_vis} Figure~\ref{fig:nakika50_demo}). As shown in figures, SESDI predict the target velocity cubes with high precision. Moreover, in Figure~\ref{fig:nakika100_demo}, we observe that SESDI could handle complicated velocity models with small salt body structures.\todo{change when better picture}

% \begin{table}[h]
% \begin{center}
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{2pt}
%  \caption{Evaluation Metrics on Nakika Data}
%  \begin{tabular}{ p{1.4cm}|p{1.2cm}|p{1.2cm}|p{1cm}|p{1cm} }
%  \hline
%  Dataset &   Method & $\ell_1$ Loss& PSNR & SSIM   \\
%  \hline\hline
% Nakika50 & SESDI & 135.2780 & 32.3479 & 0.8182   \\
% Nakika100 & SESDI & 164.9949 & 26.9546 & 0.7462   \\
%  \hline
 
% \end{tabular}\label{eval:nakika}
% \end{center}
% \end{table}






% 1. Toy datasets from FCNVMB. Our model is superior / at par with CNN and work on realistic data and not regular data required by CNN

% 2. towards realistic setting. Irregular Observations . CNN cannot be run on these

% 3. Real Nakika data : train - nakika , test - nakika part 2

% 4. Real - train nakika , test some other survey
\vspace{-0.2cm}
\section{Discussion} 
\vspace{-0.2cm}

% should be improved
%From experiments in synthetic and raw sesimic data, we have three major observations: (1) It is possible for a deep learning approach to achieve accurate seismic modeling such as VMB without seismic imaging and convolutional networks. (2) The VMB on real seismic data can be regared as an inverse problem under irregular observations  (3) The set formulation on raw seismic data improves the scalability of deep learning approaches in real SDI.  Therefore, SESDI could be considered as one of the scalable formulation that extend deep learning's application in real SDI by tackling inverse problem under irregular observations. 
The SESDI approach of breaking the task of huge property model prediction into smaller context based block prediction lets us apply deep learning successfully to the problem of sesmic inversion. From the experiments performed on synthetic and real seismic data, we observe that (1) Deep learning approach like SESDI can be successfully used to achieve accurate sesimic modelling on real scale raw seismic data. (2) Convolutions SDI are inherently flawed and unscalable to real data. We urge the community to reconsider the assumption that seismic data is image-like. (3) Formulating data as $sets$ gives us models that are robust to irregular data collection. (4) $set$ models are particularly resistant to problems like overfitting. 

The SESDI approach to Seismic data Ingestion is much more general. We believe that it would be applicable to many inverse problems under irregular observations such as 3D scene generation, medical imaging etc. 



==> approach.tex <==
\section{SESDI : Set Embedding based Seismic Data Ingestion}
\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figures/SESDI.png}
    \caption{SESDI Model Architecture}
    \label{fig:model}
\end{figure}
\subsection{Motivation and Theory}
    We discussed real acquisition in section 2.3. On this backdrop, consider a Seismic workflow for SI or VMB focusing on a particular block of subsurface in Figure \ref{fig:exgen}. For this block of interest let the collection of traces be T and its corresponding Acquisition Geometry be $A_{T}$. We have seen that $A_{T}$ is  1) notde regular 2) not consistent w.r.t different locations of block of interest. Also, the size of T might vary w.r.t the location of the block. Let F be a function that ingests the seismic data $(T, A_T)$. Let us look at the properties of F.
    \begin{itemize}
        \item F should be invariant to the order of traces in T. 
        \item F should be able to ingest data of different dimensions as size $|T|$ can vary.
    \end{itemize}
    
     These properties imply that F should treat the collection T as a $set$ of traces. In their recent paper, \cite{deepsets}, state a result for such functions F. This is stated below
     \begin{thm}
         Any function $F : X \longrightarrow R$, $X \subseteq 2^{\mathcal{X}}$ where $\mathcal{X}$ is a countable set is invariant to order of elements in X if and only if F can be written as $\rho (\Sigma_{x \in X} \phi(x))$ for appropriate functions $\rho$ and $\phi$
     \end{thm}
     Although, the results for for of $F$ when $\mathcal{X}$ is uncountable set, are not very strong \cite{deepsets}, we draw inspiration from this theoretical result to design our SESDI Architecture.
     


\subsection{SESDI Model}
For this section, let trace-aq-info(t) of a trace t be acquisition geometry associated with the trace t. Let trace-info(t) be the complete tuple containing trace-aq-info(t) and trace data t. Then the relevant raw shot gather data can be seen as a $set$ of many such trace-infos.
\begin{align*}
&\text{trace-aq-info} = (\text{source}(X,Y,Z), \text{receiver}(X,Y,Z))\\
&\text{trace-info} = (\text{trace-aq-info}, \text{trace-data})\\
&\text{raw-gather-data} = \{\text{trace-info}\}
\end{align*}
The model we use is as follows and is presented in the figure \ref{fig:model} For each trace-info, we first find embedding of trace-aq-info and trace-data via functions $\mathcal{F}_{aq}$ and $\mathcal{F}_d$ respectively. We then concatenate the two embeddings and pass it via another function $\mathcal{F}_t$ to generate the embedding for a trace-info. Then the embedding for the set of trace-infos, i.e. raw-gathers, is obtained by taking the element wise average of all the embeddings of trace-infos. 
\begin{align*}
    \text{Embedding} & (\text{trace-info}) \\
      & = \mathcal{F}_t (\mathcal{F}_{aq}(\text{trace-aq-info}) \cdot \mathcal{F}_{d}(\text{trace-data}))\\
    \text{Embedding} & ({\text{raw-gathers}}) \\
     & = \frac{1}{k} \Sigma_{i=1}^k \mathcal{F}_T (\text{trace-info}_i)
\end{align*}

%Taking average instead of sum is important as not all training samples will have equal number of trace-infos. 
This raw-gather embedding can then be further processed for specific seismic workflow objectives like SI or VMB. See Figure \ref{fig:workflow_refseis}. 

In figure \ref{fig:model}, all the functions $\mathcal{F}_t$, $\mathcal{F}_{aq}$ and $\mathcal{F}_d$ are implemented via Multi-layer perceptrons (MLPs). This is just one architecture for the functions and one can experiment with it. In our experiments on VMB we use MLP based model architecture as shown in Figure \ref{fig:model}.



% \vskip -1in
\subsection{Benefits of SESDI}




\begin{figure*}[htb]
\begin{center}
 \mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_0.jpg}
    }

\mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_3.jpg}
    }

\mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_7.jpg}
    }
\mbox{\hspace{-0.25in}
\includegraphics[width=5in]{figures/SEGSalt/bar.pdf}
    }
\end{center}

\vspace{-0.15in}
\caption{Visualization of Prediction on SEGSalt Dataset.The prediction results for U-net vs SESI model. SESI performs well even on irregularly sampled 50\% data which mimics realistic acquisition where as U-net cannot be applied on this data. }\label{fig:salt_demo}
\end{figure*}
\paragraph{Robust to varying and irregular acquisition geometry}
The SESDI model finds an embedding of each of the trace-info in raw-gathers set independent to each other and combines them in a permutation invariant manner. Hence, it does not impose any regularity or consistency restrictions on acquisition geometry and works well with varying sizes of raw-gathers. 
%Most CNN based networks require either regular acquisition geometry , listing of all possible source, reciever pairs \cite{Li_2020, Yang2019Deeplearning, inversionnet} or some feature extraction to convert the available data into regular data block \cite{semblance}. Regular Acquisition can almost never be achieved in real data gathering. Also, with reasonably sized 3D velocity blocks to predict, the area for relevant acquisition is considerably large. Number of all the possible (source, receiver) combinations even after reasonable grid quantization is very huge. These are exactly the reasons why it is difficult to apply models from current literature to real data.  Our model does not suffer from any such short-coming. Also, it does not require any kind of pre-processing and can work on raw traces. As is the case with real acquisitions, the number of traces in relevant acquisition area might vary from location to location. The model gracefully incorporates such requirements. 

\textbf{Computationally scalable to real data}
Most of the models in current literature work with 2D synthetic velocities where raw data takes a 3 dimensional form $(\text{source}_x, \text{receiver}_x, \text{time})$. Extending these models to 3D involves higher dimensional convolutions as now the data is at least 5 dimensional $(\text{source}_x, \text{source}_y, \text{receiver}_x, \text{receiver}_y, \text{time})$. These convolutions are very expensive to compute during both training and inference steps. SESDI, on the other hand , is not really affected by 2D / 3D inversion setups. The only change occurs in the dimension of trace-aq-info which has negligible effect on involved computation. Furthermore, there is even more meta-data associated with each trace. With convolutions it is impossible to fully utilize all the meta data due to increasing dimension of the convolutions. However, SESDI can easily be extended to find embeddings of this meta data and combining them into a trace-info embedding at minuscule additional cost. Hence SESDI has the potential to fully utilize entire available data.

\textbf{Does not overfit even under scarce data}
Labelled data for the seismic tasks such as  VMB or SI is generally scarce. In order to train models, generally large amounts of synthetically generated data is used to train models. SESDI is especially resistant to over-fitting due to its architecture. Every sample of size say k for training SESDI can be essentially used to generate $2^k$ samples by subsampling the data. Hence, small number of samples can be used to train complicated SESDI model. We observe this even in our experiments, where the model test results keep on improving the longer we train without over-fitting . See Figure \ref{fig:frac_overfit} 







%\subsection{Essential Components of training our model.}
%In this section, we detail some of training choices we believe are generally applicable for training our model. We train our model with ADAM \cite{adam} optimizer. We start with a small learning rate and reduce the learning rate with a factor after a fixed number of epochs. We observe that we need to train for a long time to get sufficiently good models. This might be an artifact of small initial learning rate. For example while training model on SegSaltData having 130 training samples (see Experiments), we set initial learning rate to be 1e-5 and reduce the learning rate by factor of 0.9 every 25 epochs. Also, we run for over 1000 epochs to get reasonably small training error. Also, as discussed earlier each sample has a lot of information, it is enough to set the batch size to 1 to reduce the computation for each gradient update step.

% Training Data generation for VMB
% Now we describe the process in order to generate a (raw-gathers, velocity-model) instance from the survey at hand. raw-gathers here is a subset of the raw-gather data. This survey can be a synthetically designed setup or a real survey for which we have found a good velocity model using traditional seismic processing.  The way we generate (raw-gathers, velocity-model) is shown in the figure \ref{fig:exgen}
%In order to make a training sample, we first identify a block of velocity in the area of interest. Let the width of this block be $W_v$ and depth be $D_v$. The block $W_v \times W_v \times D_v$ shown in the figure is the target block of velocity. Theoretically, all the traces in raw-gather-data might contain the information pertinent to the target velocity block. However we can use a subset of the traces to reduce the amount of data ingested per training step. The way we do this is by considering area ($W_a \times W_a$) around the velocity block shown as relevant acquisition area around the velocity block in the figure. We choose all the trace-infos such that both source and receiver lie this in region. This is a sensible way to create subset as the traces near the velocity block will be the ones most affected by it. Choice of $W_a$ will depend on how deep we want to predict. In order to predict deeper values of velocity, we would want to increase the value of $W_a$ to cover relevant traces. Let the set of traces thus obtained be $\{\text{trace-info}_i\}_{i=1}^k$ where k is the total number of traces in the subset. Here ($\{\text{trace-info}_i\}_{i=1}^k$, velocity-block) is an instance of training sample. We can generate many such samples by changing the velocity block location on the surface of the survey.


==> n1_approach.tex <==
% \newpage
\section{SESDI: Set Embedding based Seimisic Data Ingestion}
\subsection{Learning Vector Representation of Traces}


\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/data.png}
    \caption{Generating a training sample from the survey for an example Seismic Workflow of VMB. In this, we create the collection T of traces relevant to block of subsurface using an area $W_a \times W_a$ surrounding the block and choosing traces for which both source and receiver lies in this area. This is an example of how the collection of traces can be chosen.}
    \label{fig:exgen}
\end{figure}

This section introduces the distributed vector representation of seismic traces. Considering the task of velocity inversion as a running example, as shown in Figure \ref{fig:exgen}, the input of SDI is a bag of raw seismic traces with associated positions of source and receiver and the target is a 2D/3D discretized velocity matrix with uniform velocity in each partition. Each trace contains time series recording of a amplitude of pressure wave measured at receiver. For a given source and receiver location, the receiver catches the reflected waves from different depths and directions. The recorded amplitude is a superposition of all waves that reach the receiver at the same time. Hence, each trace captures information about entire subsurface and the wave reflected from distant points (depth wise or horizontal distance wise) wanes with less amplitude contributions. However, the trace data is highly redundant and correlated. In this respect, raw data is a collection of overlapping pieces of information about the entire subsurface. The challenge SESDI faces is to align information of these pieces effectively before combining them into the entire subsurface model.



In our SESDI framework, every traces is mapped to a unique vector via location-aware projection.  Formally, given a bag of location aware seismic traces $\{w_1, w_2,....,w_n\}$, where $w_i=(u_i,q_i)$ is a tuple with trace data $u$ and their acquisition geometry information $q$. We target at generating the trace embedding $\mathcal{E} (w_i)$ by 


\begin{align*}
    \mathcal{E} (w_i) 
      & = \mathcal{F}_t \left(\left[\mathcal{F}_{aq}(q_i) , \mathcal{F}_{d}(u_i)\right]\right)
\end{align*}

% Consider the task of velocity inversion as a running example. In this task the input is a bag of raw seismic traces with associated positions of source and receiver and output is a velocity model of the subsurface. We use a discretized 3D cube with uniform velocity in each partition as our target velocity model. 
% %redundancy in trace information and bag of traces
% Each trace contains time series recording of a amplitude of pressure wave measured at receiver. For a given source and receiver location, the receiver catches the reflected waves from different depths and directions. The recorded amplitude is a superposition of all waves that reach the receiver at the same time. Hence, effectively each trace captures some information about entire subsurface. Of course the wave reflected from points further away (depth wise or horizontal distance wise) wanes and the amplitude contributions lessens. However, this means the trace data is highly redundant and traces are correlated. In this respect, raw data is a collection of overlapping pieces of information about the entire subsurface. The challenge SESDI faces is to align each of this piece correctly before combining them into the entire subsurface model.


% task1 : domain change of trace and alignment.
% The domain of input trace : time series data for a location configuration) is very different from the domain of output velocity model : physical 3 dimensional space. The first goal of SESDI is to project the trace into a concept space which can be easily used to infer properties in 3 dimensional phyical domain. The information of acquisition of a trace is important to align the semantic information correctly and consistently with the physical domain. In SESDI, we acheive this aligned semantic embedding by first projecting the trace and its acquisition information into intermediate high dimensional space, combining them and projecting them in the final target embedding space. Formally, 
% \begin{align*}
%     \mathcal{E} & (\text{trace-info}) \\
%       & = \mathcal{F}_t (\mathcal{F}_{aq}(\text{trace-aq-info}) \cdot \mathcal{F}_{d}(\text{trace-data}))
% \end{align*}


In our experiments on seismic data, we use Multi layer Perceptrons (MLPs) for the functional blocks $\mathcal{F}_{aq}$, $\mathcal{F}_d$ and $\mathcal{F}_t$. In this way, every raw seismic trace is projected  into a concept space with awareness to both acquisition geometry and physical properties in the interested domain.

\subsection{Set Representation on Geometry-Aware Traces}

In this section, we present the learning approach that unify the distributed traces representation for final prediction. Due to the irregular acquisition of traces in real survey ( see Figure \ref{fig:acquisition}).  It is impossible to impose specific structural formulation such as convolution on the trace embeddings. Moreover, the number of traces varies in different interested areas, making it challenging to concatenate. 

To tackle these issues, we propose a set formulation to learn vector representation on bag of geometry-aware trace embeddings. Formally, the embedding of the interested velocity matrix is defined as:

% The acquisition of traces is highly irregular in a typical real survey( see figure \ref{fig:acquisition}). This prohibits us from imposing any structure on the acquisition and hence we have to treat raw data as a simple bag of traces. The most effective way to combine such a data is average all the aligned projections to obtain a semantic embedding of the raw data. Correct alignment of semantic embeddings is essential to support such method of combination. The larger the number of traces, the more information is contained in the semantic embedding of raw-data. Formally,
% \begin{align*}
% \mathcal{E}({\text{raw-gathers}})  = \frac{1}{k} \Sigma_{i=1}^k \mathcal{E} (\text{trace-info}_i)
% \end{align*}

\begin{align*}
\mathcal{E}({v})  = \mathcal{\rho} \left(\frac{1}{k} \Sigma_{i=1}^k \mathcal{\phi}( \mathcal{E} (w_i))\right)
\end{align*}
. Each trace embedding $\mathcal{E} (w_i)$ is first projected through a non-linear mapping $\phi$. Then the average of projected trace vectors are used as features for the final non-linear mapping  $\rho$. The SESDI architecture implements $\rho$ and $\phi$ as MLPs. The overview of SESDI models are shown in Figure \ref{fig:model}
\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figures/SESDI.png}
    \caption{SESDI Model Architecture}
    \label{fig:model}
\end{figure}




% \todo{can we elaborate this connection deep set model more}
The set representation of SESDI is associated with a theoretical result in Deep learning \cite{deepsets}. The statement of the theorem as is, is stated below:
     \begin{thm}
         Any function $F : X \longrightarrow R$, $X \subseteq 2^{\mathcal{X}}$ where $\mathcal{X}$ is a countable set is invariant to order of elements in X if and only if F can be written as $\rho (\Sigma_{x \in X} \phi(x))$ for appropriate functions $\rho$ and $\phi$
     \end{thm}
There exists conjecture that such a result is true even when $\mathcal{X}$ is not countable. As we use MLPs for $\rho$ in our case without passing the information about number of traces to it, we explicitly use a average instead of sum as suggested by the theorem. 


In practice, the SESDI is trained through a subsampling strategy. Given every bag of traces $W=\{w_1, w_2,....,w_n\}$, we uniformly sample a subset $S_j\subseteq W$ and perform training on various subsets. Meanwhile, in the testing, we also randomly subsample the testing bag of traces and perform inference. The major advantages of this strategy are: (1) we overcome the limitation of original dataset scale and enable training with better generalization on large but limited seismic training samples. (2)  the SESDI is trained on a more irregular setting and becomes more scalable to real SDI tasks. (3) the subsampling on inference phase reduce the overhead in matrix computation, enabling more efficient deployments on environmental applications. 
% \todo{how to introduce training data generation section}

% \vskip -1in
\subsection{Benefits of SESDI}




\begin{figure*}[htb]
\begin{center}
 \mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_0.jpg}
    }

\mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_3.jpg}
    }

\mbox{\hspace{-0.25in}
\includegraphics[width=5.3in]{figures/SEGSalt/Vis_7.jpg}
    }
\mbox{\hspace{-0.25in}
\includegraphics[width=5in]{figures/SEGSalt/bar.pdf}
    }
\end{center}

\vspace{-0.15in}
\caption{Visualization of Prediction on SEGSalt Dataset.The prediction results for U-net vs SESI model. SESI performs well even on irregularly sampled 50\% data which mimics realistic acquisition where as U-net cannot be applied on this data. }\label{fig:salt_demo}
\end{figure*}
\paragraph{Robust to varying and irregular acquisition geometry}
The SESDI model finds an embedding of each of the trace-info in raw-gathers set independent to each other and combines them in a permutation invariant manner. Hence, it does not impose any regularity or consistency restrictions on acquisition geometry and works well with varying sizes of raw-gathers. 
%Most CNN based networks require either regular acquisition geometry , listing of all possible source, reciever pairs \cite{Li_2020, Yang2019Deeplearning, inversionnet} or some feature extraction to convert the available data into regular data block \cite{semblance}. Regular Acquisition can almost never be achieved in real data gathering. Also, with reasonably sized 3D velocity blocks to predict, the area for relevant acquisition is considerably large. Number of all the possible (source, receiver) combinations even after reasonable grid quantization is very huge. These are exactly the reasons why it is difficult to apply models from current literature to real data.  Our model does not suffer from any such short-coming. Also, it does not require any kind of pre-processing and can work on raw traces. As is the case with real acquisitions, the number of traces in relevant acquisition area might vary from location to location. The model gracefully incorporates such requirements. 

\textbf{Computationally scalable to real data}
Most of the models in current literature work with 2D synthetic velocities where raw data takes a 3 dimensional form $(\text{source}_x, \text{receiver}_x, \text{time})$. Extending these models to 3D involves higher dimensional convolutions as now the data is at least 5 dimensional $(\text{source}_x, \text{source}_y, \text{receiver}_x, \text{receiver}_y, \text{time})$. These convolutions are very expensive to compute during both training and inference steps. SESDI, on the other hand , is not really affected by 2D / 3D inversion setups. The only change occurs in the dimension of trace-aq-info which has negligible effect on involved computation. Furthermore, there is even more meta-data associated with each trace. With convolutions it is impossible to fully utilize all the meta data due to increasing dimension of the convolutions. However, SESDI can easily be extended to find embeddings of this meta data and combining them into a trace-info embedding at minuscule additional cost. Hence SESDI has the potential to fully utilize entire available data.

\textbf{Does not overfit even under scarce data}
Labelled data for the seismic tasks such as  VMB or SI is generally scarce. In order to train models, generally large amounts of synthetically generated data is used to train models. SESDI is especially resistant to over-fitting due to its architecture. Every sample of size say k for training SESDI can be essentially used to generate $2^k$ samples by subsampling the data. Hence, small number of samples can be used to train complicated SESDI model. We observe this even in our experiments, where the model test results keep on improving the longer we train without over-fitting . See Figure \ref{fig:frac_overfit} 







%\subsection{Essential Components of training our model.}
%In this section, we detail some of training choices we believe are generally applicable for training our model. We train our model with ADAM \cite{adam} optimizer. We start with a small learning rate and reduce the learning rate with a factor after a fixed number of epochs. We observe that we need to train for a long time to get sufficiently good models. This might be an artifact of small initial learning rate. For example while training model on SegSaltData having 130 training samples (see Experiments), we set initial learning rate to be 1e-5 and reduce the learning rate by factor of 0.9 every 25 epochs. Also, we run for over 1000 epochs to get reasonably small training error. Also, as discussed earlier each sample has a lot of information, it is enough to set the batch size to 1 to reduce the computation for each gradient update step.

% Training Data generation for VMB
% Now we describe the process in order to generate a (raw-gathers, velocity-model) instance from the survey at hand. raw-gathers here is a subset of the raw-gather data. This survey can be a synthetically designed setup or a real survey for which we have found a good velocity model using traditional seismic processing.  The way we generate (raw-gathers, velocity-model) is shown in the figure \ref{fig:exgen}
%In order to make a training sample, we first identify a block of velocity in the area of interest. Let the width of this block be $W_v$ and depth be $D_v$. The block $W_v \times W_v \times D_v$ shown in the figure is the target block of velocity. Theoretically, all the traces in raw-gather-data might contain the information pertinent to the target velocity block. However we can use a subset of the traces to reduce the amount of data ingested per training step. The way we do this is by considering area ($W_a \times W_a$) around the velocity block shown as relevant acquisition area around the velocity block in the figure. We choose all the trace-infos such that both source and receiver lie this in region. This is a sensible way to create subset as the traces near the velocity block will be the ones most affected by it. Choice of $W_a$ will depend on how deep we want to predict. In order to predict deeper values of velocity, we would want to increase the value of $W_a$ to cover relevant traces. Let the set of traces thus obtained be $\{\text{trace-info}_i\}_{i=1}^k$ where k is the total number of traces in the subset. Here ($\{\text{trace-info}_i\}_{i=1}^k$, velocity-block) is an instance of training sample. We can generate many such samples by changing the velocity block location on the surface of the survey.




==> tab_all_res_2.tex <==
\begin{table*}[]
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Datasets &
  \multicolumn{3}{l|}{SEGSalt} &
  \multicolumn{3}{l|}{RS-SEGSalt} &
  &
  GulfM-10 &
  GulfM-20\\ \hline
Models          & l1     & PSNR  & SSIM &      & PSNR  & SSIM & Models  & SESDI & SESDI  \\ \hline
U-Net           & 196.82 & 14.64 & 0.45 & -    & -    & -   & l1    &135.27   & 164.99    \\ \hline
Set-Transformer & 232.78 & 14.21 & 0.40 & 294.76 & 14.90 & 0.34 & PSNR  & 32.34   & 26.95     \\ \hline
SESDI &
  \textbf{163.77} &
  \textbf{16.65} &
  \textbf{0.47} &
  \textbf{162.79} &
  \textbf{16.68} &
  \textbf{0.41} &
  SSIM &
  0.82  &
  0.75 
 \\ \hline
\end{tabular}
}
\vspace{-0.1cm}
\caption{Summary of Results of SESDI and baselines on all the four datasets.}
\label{tab:all-results}
\vspace{-0.5cm}
\end{table*}
